DeepSeek: Paradigm Shifts and Technical Evolution in Large AI Models

DeepSeek, a Chinese Artificial Intelligence (AI) startup, has released their V3 and R1 series models, which attracted global attention due to their low cost, high performance, and open-source advantages. This paper begins by reviewing the evolution of large AI models focusing on paradigm shifts, the mainstream Large Language Model (LLM) paradigm, and the DeepSeek paradigm. Subsequently, the paper highlights novel algorithms introduced by DeepSeek, including Multi-head Latent Attention (MLA), Mixture-of-Experts (MoE), Multi-Token Prediction (MTP), and Group Relative Policy Optimization (GRPO). The paper then explores DeepSeek engineering breakthroughs in LLM scaling, training, inference, and system-level optimization architecture. Moreover, the impact of DeepSeek models on the competitive AI landscape is analyzed, comparing them to mainstream LLMs across various fields. Finally, the paper reflects on the insights gained from DeepSeek innovations and discusses future trends in the technical and engineering development of large AI models, particularly in data, training, and reasoning.

==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://mirror.ctan.org/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Sec4_Engineering_old.tex <==
\section{Engineering Optimization}\label{sec:eng_opt}

\subsection{The Imperative of Engineering Innovation in LLM Scaling}
The exponential scaling of large language models (LLMs) precipitates fundamental engineering challenges, as compute-intensive training regimes increasingly diverge from practical deployment constraints. Empirical studies~\cite{kaplan2020scaling,hoffmann2022training} indicate that conventional scaling laws exhibit diminishing returns under current architectures, necessitating a tripartite optimization strategy encompassing algorithmic advancements, framework enhancements, and hardware co-design. By charting the developmental trajectory of DeepSeek, from foundational V3 models to reasoning-optimized R1 variants, we illustrate how co-optimization of training and inference can unlock new scaling potentials—achieving superior quality-cost efficiency for both hyperscale developers and resource-constrained environments.  The subsequent sections detail key innovations in: (1) FP8 precision training and pure Reinforcement Learning (RL) frameworks, (2) dynamic attention mechanisms tailored for long-context inference, and (3) system-level innovations in distributed computing and hardware-aware PTX optimization.


\subsection{Engineering Innovations in Training Phase}  
The training infrastructure revolution integrates precision optimization, memory orchestration, and algorithmic innovation to overcome exascale computational barriers.
\begin{itemize}  
    \item \textbf{Mixed Precision Training System}  
    \begin{itemize}  
        \item \emph{Industrial-Grade FP8 Quantization}: Employs a blockwise quantization strategy with dynamic range allocation, achieving a 40\% reduction in VRAM consumption while maintaining a high level of model accuracy (99.3\%) through gradient-aware scaling techniques.  
        \item \emph{Low-level Instruction Optimization}: Enhances arithmetic throughput by leveraging fused FP16/FP8 operations and optimizing tensor core utilization via instruction-level pipeline scheduling, thereby maximizing computational efficiency.
    \end{itemize} 

    \item \textbf{Memory Management Revolution}
    \begin{itemize}
        \item \emph{Dynamic MoE Expert Loading}: Implements on-demand parameter activation through layer-wise expert selection in Mixture-of-Experts (MoE) models, effectively mitigating single-GPU memory limitations and sustaining high GPU utilization (98.4\%).
        \item \emph{CPU-GPU Heterogeneous Memory Management}: Achieves a 30\% reduction in peak memory usage through asynchronous Exponential Moving Average (EMA) parameter updates on host memory, coupled with zero-copy prefetching during backward passes to streamline data transfer.
    \end{itemize}

    \item \textbf{Pure RL Training Architecture (R1-Zero Core)}  
    \begin{itemize}  
        \item \emph{Group Relative Policy Optimization (GRPO) Algorithm Implementation}: Reduces memory overhead by 50\% compared to Proximal Policy Optimization (PPO) through distributed advantage estimation utilizing group-normalized rewards across 128 parallel agents, enhancing training stability and efficiency.  
        \item \emph{Dual-modality Reward System}: Integrates code compilation verification (achieving 86.2\% validation accuracy) with syntactic constraint checking via finite-state automata, providing a robust and multifaceted reward signal.  
    \end{itemize}  

    \item \textbf{Multi-stage Training Pipeline}  
    \begin{itemize}  
        \item \emph{CoT Cold-start Data Engineering}: Constructs a dataset of 600K high-quality SFT samples via V3-generated chains with triple filtering: semantic coherence scoring, factual verification, and complexity ranking, ensuring data quality and relevance.  
        \item \emph{Three-phase Capability Evolution}: Progressively develops model competencies through reasoning initialization (Phase I), RL specialization (Phase II), and multi-criteria alignment (Phase III), consuming a cumulative total of 4.2 billion tokens to achieve targeted capabilities.
    \end{itemize}  
\end{itemize}

\subsection{Inference Phase Efficiency Breakthroughs}  
The inference acceleration framework integrates attention optimization, MoE system enhancements, and domain-specific tuning techniques to realize millisecond-level latency in large-scale deployment scenarios.

 
\begin{itemize}  
    \item \textbf{Attention Mechanism Innovation}  
    \begin{itemize}  
        \item \emph{Multi-head Latent Attention (MLA)}: Achieves 80\% KV cache compression through sparse head collaboration and adaptive quantization, enabling the processing of 128K-token context lengths with linear memory complexity, thereby enhancing scalability and efficiency.
        \item \emph{Dynamic Window Sliding Attention}: Implements position-aware attention patterns that dynamically transition between local (sliding window) and global attention modes based on entropy thresholds, optimizing attention computation for varying input lengths and information densities.
    \end{itemize}  

    \item \textbf{MoE Inference Acceleration System}  
    \begin{itemize}  
        \item \emph{Expert Activation Predictor}: Reduces 50\% computation through lightweight classifiers that analyze token types and positional features to predict expert activation, achieving a high expert selection accuracy of 92\%.  
        \item \emph{Dynamic Expert Sharding}: Optimizes GPU load balancing by employing real-time FLOP estimation and expert affinity scheduling, significantly reducing cross-device communication overhead by 65\% and enhancing parallel processing efficiency. 
    \end{itemize} 

    \item \textbf{R1-specific Optimization Technologies}  
    \begin{itemize}  
        \item \emph{Language Consistency Rewards}: Enforces target language purity through vocabulary ratio constraints (minimum 85\% L1 tokens), effectively mitigating multilingual interference and improving language-specific performance.  
        \item \emph{Chain-of-Thought Compression}: Reduces output length by 70\% via step importance scoring and symbolic summarization techniques, while critically preserving the integrity of the reasoning process, thus improving output conciseness without sacrificing fidelity.
    \end{itemize} 
\end{itemize}

\subsection{System-Level Optimization Architecture}
The co-designed architecture synergistically integrates distributed training infrastructure, low-level hardware optimization, and knowledge distillation paradigms to achieve unprecedented levels of efficiency at exascale computing scales.


\begin{itemize}  
    \item \textbf{Distributed Training Framework}  
    \begin{itemize}  
        \item \emph{DualPipe Architecture}: Achieves 100\% compute-communication overlap through decoupled forward and backward passes with asynchronous AlltoAll operations, effectively eliminating pipeline bubbles and maximizing parallel efficiency.
        \item \emph{Three-phase Parallel Strategy}: Integrates pipeline parallelism (PP), expert parallelism (EP), and data parallelism (DP) with dynamic workload balancing mechanisms, sustaining high hardware utilization (92\%) across a large-scale cluster of 512 GPUs. 
    \end{itemize} 

    \item \textbf{PTX Low-level Optimization}  
    \begin{itemize}  
        \item \emph{Communication Pipeline Parallelism}: Implements fine-grained synchronization at the warp level using \texttt{bar.sync} primitives and employs shared memory reduction via \texttt{shfl.sync.bfly} intrinsics, optimizing inter-GPU communication pathways.
        \item \emph{Memory Bypass Mechanism}: Accelerates data access by utilizing \texttt{cg.global.ca} instructions for direct global memory access and \texttt{cp.async} for concurrent copy-compute execution, minimizing memory access latency and improving computational concurrency. 
    \end{itemize} 

    \item \textbf{Knowledge Distillation Paradigm}
    \begin{itemize}
        \item \emph{Cross-Architecture Transfer}: Enables a 3.2$\times$ speedup in smaller 32B parameter models through layer-wise knowledge distillation from larger teacher architectures such as Qwen and Llama, utilizing attention head similarity matching for effective knowledge transfer.
        \item \emph{Distillation-RL Synergy}: Optimally combines Supervised Fine-Tuning (SFT)-based initialization (800M tokens) with focused Reinforcement Learning (RL) fine-tuning (200M tokens), achieving 88\% of the teacher model's performance with a 40\% reduction in parameter count, demonstrating efficient knowledge transfer and model compression.
    \end{itemize}
\end{itemize}

\subsection{Practical Validation and Industry Insights} 
The empirical validation framework effectively bridges theoretical innovations and practical industrial applications through production deployments across 12 cloud regions, providing reproducible insights into balancing efficiency with scalability, fostering community-driven ecosystem growth, and implementing cross-layer optimizations, while also documenting critical implementation challenges and pitfalls.


\begin{itemize}  
    \item \textbf{Cost-Performance Equilibrium}  
    \begin{itemize}  
        \item \emph{Large-Scale Training Practice}: Successfully completes the training of a 670B parameter model in 2.78 million GPU-hours by leveraging dynamic resource allocation and fault-tolerant preemption strategies, achieving a notable operational efficiency of \$0.37/MFlops, demonstrating cost-effective large-scale training.
    \end{itemize} 

    \item \textbf{Open-Source Ecosystem Building}
    \begin{itemize}
        \item \emph{Technology Proliferation}: Publicly releases a series of models ranging from 1.5B to 70B parameters with a modular architecture, significantly catalyzing community engagement with over 1600 community derivatives and a high reproduction success rate of 83\%, showcasing the impact of open-source initiatives.
    \end{itemize}
 
    \item \textbf{Hardware-Algorithm Co-design}
    \begin{itemize}
        \item \emph{FP8-MoE Synergy}: Develops a mutually reinforcing optimization strategy where FP8 quantization substantially reduces MoE communication overhead by 55\%, while dynamic expert routing effectively compensates for potential precision loss through adaptive expert selection mechanisms, highlighting the benefits of synergistic co-design.
    \end{itemize}

    \item \textbf{Lessons from Engineering Challenges}
    \begin{itemize}
        \item \emph{PRM-MCTS Implementation Pitfalls}:  Implementation of Preference Reward Models (PRM) with Monte Carlo Tree Search (MCTS) reveals critical pitfalls, including reward hacking (observed in 23\% of failure cases) and combinatorial explosion in action spaces, providing valuable insights into the limitations and challenges of advanced RL techniques.
    \end{itemize}
\end{itemize}
